A Survey on Scenario-Based Testing for Automated Driving Systems in High-Fidelity Simulation

Automated Driving Systems (ADSs) have seen rapid progress in recent years. To ensure the safety and reliability of these systems, extensive testings are being conducted before their future mass deployment. Testing the system on the road is the closest to real-world and desirable approach, but it is incredibly costly. Also, it is infeasible to cover rare corner cases using such real-world testing. Thus, a popular alternative is to evaluate an ADS's performance in some well-designed challenging scenarios, a.k.a. scenario-based testing. High-fidelity simulators have been widely used in this setting to maximize flexibility and convenience in testing what-if scenarios. Although many works have been proposed offering diverse frameworks/methods for testing specific systems, the comparisons and connections among these works are still missing. To bridge this gap, in this work, we provide a generic formulation of scenario-based testing in high-fidelity simulation and conduct a literature review on the existing works. We further compare them and present the open challenges as well as potential future research directions.

==> body/9backup.tex <==
\appendices
\section{Evolutionary Algorithm By Individual Work}

\begin{algorithm}
    \scriptsize
    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}
    
    \Input{$D$: search space, $G$: maximum number of generations, $initialize(D)$: generate the initial scenario vectors, $select(S)$: select the parents to do cross-over from a set $S$, $parent\_select(D, S, R)$: select parent scenario vectors, $crossover(S)$: apply cross-over to a set of chosen scenario vectors $mutate(S)$: apply mutation to a set of chosen scenario vectors,
    $seed\_select(D, S, R)$: select seed scenario vectors to run, $evaluate(S)$: evaluate the fitness values of a set of scenario vectors and return the results.}
    % \Output{}
    
    $S = initialize(D)$\;
    $R = evaluate(S)$\;
    
    \While {$i < G$}{
        $i+= 1$\;
        
        $S = parent\_select(D, S, R)$\;
        $S = crossover(S)$\;
        $S = mutate(S)$\;
        $S = seed\_select(S)$\;
        $R = evaluate(S)$\;
    }
    
    % \Return $x$

    \caption{\textbf{\small{Evolutionary Algorithm}}}
    \label{alg:ea}
\end{algorithm}


\cite{kluck19} applies a standard GA with TTC as its fitness function to find the most critical scenario (based on min TTC) for an AEB in a car following scenario in \vtd.

\cite{asfault19} applies a standard GA to maximally find wrong-lane scenarios for the lane following functionality of BeamNG.AI and DeepDriving in \beamngtech. Its search space parametrizes road networks consisting of road segments, each of which consists of turn angle and length. The algorithm uses the ego car's maximum deviation from the lane center as the fitness function to promote finding scenarios in which the ego car drives off the road. It sets $mutation$ to randomly replacing road segments of a road network with new ones and $crossover$ to recombine or redistribute road segments. Invalid $mutation$ and $crossover$ have an increasing probability of being given up and decreasing probability of being retried. Finally, the algorithm is evaluated by counting the number of off-road accidents found.

\cite{nsga2sm16} tries to find the most critical as well as responsible scenarios for an FCW in a pedestrian crossing street scenario in \prescan. It uses a variant of NSGA2\cite{nsga202}, which is a multi-objective GA with binary tournament selection for $select$, simulated binary crossover\cite{deb95} for $crossover$, and a polynomial mutation for $mutate$. Before running NSGA2, the algorithm trains three shallow neural networks for predicting a scenario vector's three objective values based on some pre-collected running data. The three objectives are ego car's speed at collision, min distance for the pedestrian to the FCW's warning area, and min TTC to the pedestrian. At each generation, it runs NSGA2 to generate candidate scenario vectors and leverage the NNs to predict their objective values. A confidence interval based on all the simulated instances so far is also calculated for each objective function. Scenario vectors with the highest ranks  and larger predicted objective values (after adding a confidence interval for each objective) than the previous best ones are chosen to run. The algorithm is evaluated based on the hypervolume of the scenario vectors at the Pareto front.

\cite{nsga2dt18} tries to find more as well as the most critical and responsible scenarios of an AEB system in \prescan. Similar to \cite{nsga2sm16}, the algorithm also runs NSGA2 as a subroutine for multiple rounds. It uses a 3-dimensional fitness function consisting of min distance to pedestrian, speed of ego car at collision, and confidence of the system's detection. In particular, after each generation finishes, it fits a decision tree(DT) classifier over all simulated instances so far based on if they induce the critical and responsible scenarios. In the next round, only scenario vectors falling into the critical leaves of the DT will be chosen. The use of a DT classifier increases the convergence speed and enables the results to be more interpretable. In particular, for a leaf consisting of mostly critical scenarios, most scenario vectors falling into that leaf's region are likely to be critical. The proposed method is evaluated based on the number of critical scenarios with distinct scenario vectors and the hypervolume/generational distance/spread of the most critical ones at the Pareto front.

\cite{fitest18} tries to maximally identify unsafe behaviors (e.g.collision, failure to respect a stop sign/speed limit) caused by the integration component of two ADAS systems in \prescan. The algorithm uses a variant of MOSA \cite{mosa15} which is another multi-objective genetic algorithm. Since the aim is to find integration-induced errors, the fitness function is designed to promote branch coverage of the integration component, increase failure distance of the entire system output, and increase unsafe overriding distance. The algorithm is evaluated based on the number of integration-induced errors counted based on subjective judgment.

\cite{autofuzz21} proposes another variant of NSGA2 to find diverse, critical/wrong lane scenarios for PID and LBC in several NHTSA pre-crash report\cite{precrash07} inspired scenarios in \carla. Unlike NSGA2, which is a multi-objective GA, \cite{autofuzz21} uses a weighted sum of three objectives for finding critical and wrong lane scenarios, respectively. The former uses min distance to another object, ego car's speed at collision, and another object's min distance to its front camera view. The latter uses ego car's max deviation from lane center and min distance to a wrong lane and sidewalk. At each generation, the algorithm repetitively uses regular routines of NSGA2 to generate candidate scenario vectors and make sure they are further than a user-specified threshold from each other and the already found critical scenario vectors so far. The reason for the filtration is to promote the diversity of the scenario vectors in the search space. It then trains a binary shallow neural network classifier to predict if a scenario vector will lead to an accident (e.g., collision or going the wrong lane) and ranks the candidate scenario vectors based on the NN's confidence in them. Next, it applies a constrained gradient-guided mutation to mutate the scenario vectors to make them more likely to cause accidents. The method is evaluated based on how many distinct scenario vectors are found that cause critical or wrong lane scenarios. Two critical scenario vectors are considered distinct if they are a certain distance away.

\cite{fusionfuzz21} also uses a variant of NSGA2 to find avoidable, fusion-induced critical scenarios in a scenario during which NPC vehicles are constantly changing lanes in \carla. It designs a special term: the percentage of time steps in which the fusion component makes terrible decisions. The fusion component makes a wrong decision when its fused prediction is inaccurate even though at least one of its upstream predictions from multiple sensors is accurate. \cite{fusionfuzz21} counts the number of such special scenario vectors found based on the number of distinct coverage of the ego car's speed-spatial trajectory during simulation.

\cite{avfuzzer20} aims to find diverse, critical scenarios of \apollo in a scenario during which NPC vehicles are constantly changing lanes in \svl. It consists of many rounds. Each has a global GA search step and a local GA search step. The global search step aims to promote diversity, and the local search step aims to promote criticality. The fitness function is the min distance to any NPC vehicle subtracted by the min stopping distance of the ego car. The $initialize$ in the global GA search samples scenario vectors with the largest average distance from previously run scenario vectors. The rest is similar to a regular GA. When the fitness function becomes stable, it chooses the most critical scenario vector and applies the local search. It should be noted that, unlike the previous work, both $crossover$ and $mutate$ apply at the level of NPC vehicle associated parameters. It is not clear if this provides advantages over the regular routines, which apply $crossover$ and $mutate$ at the level of each field. Lastly, the critical scenarios are counted based on subjective judgment.

\cite{asf21} tries to find diverse, critical scenarios of \apollo in a regular urban driving scenario in \svl. It applies a GA with a customized $mutate$ with four specially designed operations (arithmetic, flip, random, and insert). Besides, it does not use $crossover$. Regarding the fitness function, in addition to a min distance term, it has a term to diversify an ego car's trajectory coverage during simulations. \cite{asf21} also categorizes the critical scenarios counting based on subjective judgment.

\cite{tang321} aims to find more critical scenarios for \apollo in \svl. It first categorizes routes from a map based on a junction lane coverage metric and then chooses the representatives from each category as the routes to run on. Each representative applies GA with the min distance as the objective function to further search for the additional critical scenario-inducing parameters (in particular, the locations and speed of several NPC vehicles). \cite{tang321} counts the number of critical scenarios found based on subjective judgment.

\cite{bussler20} applies DE to find severe critical scenarios for an unknown proprietary controller in a left turn scenario with both crossing vehicle and pedestrian in \vtd. The key difference between DE and GA is that DE samples three scenario vectors, applies the first two's difference to the third, and selects the third one as a parent paired with the scenario vector from the last generation. It is not clear if DE has any superiority over GA for critical scenario finding. Both the fitness function and the evaluation metric use min distance and min TTC.





\section{Simulated Annealing by Individual Work}
Simulated Annealing (SA) is another popular method. It is similar to EA, with the key difference being that it does not have $crossover$ and only uses $mutate$ to generate new scenario vectors from the previous ones. It replaces the original scenario vector with the mutated one if the mutated vector has a better fitness score. Otherwise, it will make the replacement with a certain probability based on the fitness difference.

\cite{kluck219} tries to find a critical scenario for an AEB in a car following with pedestrian crossing street scenario in \vtd using the shortest time. It uses a standard SA with min TTC as the objective function.

\cite{tuncali18} aims to find more critical, responsible scenarios for a customized CNN follower in \webots. Its $initialize$ samples from the search space based on covering array, which is a minimal number of test cases such that any t-way combination of test parameters exist\cite{Hartman2005}, for greater coverage. It then applies SA with the objective function being a weighted sum of the ego car's speed, min NPC object's distance to ego car's view, and min distance to any NPC object.

\cite{simatav20} applies SA to find more scenarios that violate a subset of requirements for a customized multi-sensor trajectory follower in three scenarios in \webots. It also uses covering array for $initialize$. The objective function is based on a chosen subset of five requirements discussed in \Cref{sec:property}.



\section{Deep Reinforcement Learning (for Special Scenario Search) by Individual Work}
Existing work usually applies Deep Reinforcement Learning (DRL) to learn a policy for an NPC vehicle or several NPC vehicles. The scenarios become more critical (along with other properties) over time. Therefore, actor-critic architecture is usually adopted. It uses two NNs for policy function and value function, respectively. 

\cite{kuutti20} uses Advantage Actor-Critic(A2C)\cite{a2c16} to find critical scenarios for two end-to-end controllers in a car following scenario in \carmaker. It designs the reward function to be the ego car's min time headway. The state space is based on the ego car velocity, acceleration, relative velocity, and time headway with the leading NPC vehicle, and the action is the leading NPC's longitudinal acceleration.

\cite{failmaker-advrl19} uses Multi-Agent Deep Deterministic Policy Gradient (MADDPG)\cite{maddpg17} in which agents learn a centralized critic based on the observations and actions of all the agents. It aims to find more critical, natural scenarios for a rule-based controller in a regular urban driving scenario in \airsim. At time step $t$, each NPC vehicle $i$ has a reward function depending on its distance to a pre-specified reference trajectory, its velocity, and its contribution to the ego car's failure. To estimate the contribution, the scenario with different subsets of K NPC vehicles will be rerun. The rerun results and the NPC i's distance to the ego car at $t$ will be used to calculate its contribution value. The state is based on the locations of all vehicles, and the action space consists of each NPC vehicle's distance to a reference trajectory.

\cite{chen21} uses ensemble DDPG to find diverse, rule-following, critical scenarios for two ALC2 in \carla. Each adversary agent (including all the NPC vehicles) has a reward equal to the weighted sum of negative ego car reward and the rule obedience reward (penalized if the NPC violates any traffic laws). The state space consists of the location of the ego car, and longitudinal position and speed of the NPC vehicles. The action space is the acceleration of the NPC vehicles. The algorithm then applies DP-Means for clustering of DNN in the ensemble to find distinct scenarios.
